SkyByte: Architecting an Efficient Memory-Semantic CXL-based SSD with OS and Hardware Co-design

The CXL-based solid-state drive (CXL-SSD) provides a promising approach towards scaling the main memory capacity at low cost. However, the CXL-SSD faces performance challenges due to the long flash access latency and unpredictable events such as garbage collection in the SSD device, stalling the host processor and wasting compute cycles. Although the CXL interface enables the byte-granular data access to the SSD, accessing flash chips is still at page granularity due to physical limitations. The mismatch of access granularity causes significant unnecessary I/O traffic to flash chips, worsening the suboptimal end-to-end data access performance. In this paper, we present SkyByte, an efficient CXL-based SSD that employs a holistic approach to address the aforementioned challenges by co-designing the host operating system (OS) and SSD controller. To alleviate the long memory stall when accessing the CXL-SSD, SkyByte revisits the OS context switch mechanism and enables opportunistic context switches upon the detection of long access delays. To accommodate byte-granular data accesses, SkyByte architects the internal DRAM of the SSD controller into a cacheline-level write log and a page-level data cache, and enables data coalescing upon log cleaning to reduce the I/O traffic to flash chips. SkyByte also employs optimization techniques that include adaptive page migration for exploring the performance benefits of fast host memory by promoting hot pages in CXL-SSD to the host. We implement SkyByte with a CXL-SSD simulator and evaluate its efficiency with various data-intensive applications. Our experiments show that SkyByte outperforms current CXL-based SSD by 6.11X, and reduces the I/O traffic to flash chips by 23.08X on average. SkyByte also reaches 75% of the performance of the ideal case that assumes unlimited DRAM capacity in the host, which offers an attractive cost-effective solution.

==> revision_log.tex <==
% \clearpage
\onecolumn
\thispagestyle{plain}
\pagestyle{plain}

\pagenumbering{arabic}

% \setstretch{0.9}

\centerline{\LARGE \textbf{Revision Logs of \pname}}
\vspace{3ex}
\noindent {\large \hlcommon{\textbf{Common Concerns}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Evaluation Baseline (Reviewer-A-D-E-F)}

We added \pname{}-CP in $\S$\ref{sec:eval}, which only enables the coordinated context switch mechanism and the adaptive page migration.
% This is a similar but more competitive baseline compared to the traditional swapping-based OS paging, which leverages host DRAM as a cache and uses context switches to hide I/O latency.
This baseline reflects the performance of leveraging host DRAM as a cache and using context switches to hide I/O latency, similar to the idea of the traditional OS page swapping. We did not directly compare \pname{} with OS page swapping since it suffers from significant swapping overhead, and \pname{}-CP always performs better than OS page swapping in our experiments.
\vspace{1ex}

As shown in Figure~\mbox{\ref{fig:eval_e2e_perf}} and Figure~\mbox{\ref{fig:eval_write_traffic}}, \pname{}-CP improves the performance over \basename{} by 2.79$\times$ on average. With the write log design in SSD DRAM, \pname{}-Full further outperforms \pname{}-CP by 1.64$\times$ on average.
% We do not compare with the traditional OS swapping directly because the CXL-based SSD functions as part of the main memory rather than a storage device.
\vspace{1ex}

We also added $\S$\ref{sec:eval_comparison} and Figure~\mbox{\ref{fig:comparision_tiered}} to evaluate \pname{}'s performance when integrating the page migration optimizations from prior studies on tiered memory systems, including TPP~\cite{tpp:asplos2023} and AstriFlash~\cite{AstriFlash}.
\pname{} outperforms these approaches by up to 4.95$\times$ (1.75$\times$ on average).
Compared to TPP, \pname{} leverages the SSD controller to track page hotness more precisely than the periodic sampling approach in TPP.
Compared to AstriFlash, \pname{} utilizes the host DRAM more efficiently since it only promotes hot pages and effectively uses the host DRAM as a fully associative cache, while AstriFlash relies on on-demand paging and manages the host DRAM as a set-associative cache.
\pname{} also benefits additionally from the write log in SSD DRAM.
% \pname{}'s CXL-aware SSD DRAM management techniques (i.e., the coordinated context switch and the write log design) can benefit software-based CXL memory systems (like TPP) on CXL-SSD.

% We first added the \textbf{\pname-CP} baseline in $\S$\ref{sec:exp_setup}, which refers to \mbox{\basename{}} with both \mbox{\pname{}'s} coordinated context switch mechanism and adaptive page migration. In a way, \pname-CP represents a projection of the traditional swapping-based OS storage management approach onto the management of CXL-SSDs, enabled by \pname's design. In this context, \pname's context switch mechanism serves a role similar to the OS's page fault mechanism, and host main DRAM is also similarly utilized as a cache for Flash at page granularity. 


% We added a new subsection $\S$\ref{sec:eval_comparison} to compare \pname with other tiered memory management approaches. We added the \textbf{\pname-CT} and \textbf{\pname-CWT} baselines where the proposed adaptive page migration mechanism is replaced with the page placement strategy from TPP\cite{tpp:asplos2023}, which is the state-of-the-art software solution for CXL-enabled tiered memory systems.

% Finally, we added the \textbf{AstriFlash-CXL} as another baseline, where the host DRAM is set as a 4KB-granularity hardware-managed set associative cache of the SSD.

% CXL memory appears to a system as a CPU-less NUMA node, it appears like the main memory. 

% Justify Base-CSSD

% AstriFlash, intrinsic CXL property?

% but in some case it could be represented using \pname-CP, \pname-CP should be better than traditional pagefault-based OS swapping approach.
\vspace{1ex}



% \item \textbf{Limited Novelty of the Idea of the Switch-on-miss Approach}
\item \textbf{Research Contributions (Reviewer A-B)}

Compared to prior works, \pname made the following main research contributions: (1) We thoroughly examine the bottlenecks of CXL-based SSDs, and identify that the tail latency of SSDs causes severe processor pipeline stalls, leading to both performance degradation and underutilization of CPU and SSD bandwidth. (2) We propose an OS and hardware co-design approach to hide long flash latency with thread-level parallelism (context switching).
(3) We recognize that a coordinated context switch mechanism, rather than the direct switch-on-miss method used in previous studies, is necessary to optimize CXL-SSD performance. This is because the host CPU is unaware of the internal state of the SSD and whether a CXL-SSD memory access latency is long enough. Therefore, \pname enables the SSD controller to decide whether to trigger a context switch based on accurate predictions of access latencies. (4) We leverage the long coalescing window of a cache-line granular write log to address the granularity mismatch issue of CXL-SSD and significantly reduce the flash write traffic. 

% (3) We propose a practical OS and hardware co-design by utilizing one of the reserved opcodes in the CXL.mem protocol to indicate context switch requests and extending the CPU’s default exception handling mechanism to support this new context switch. Our approach requires minimal modifications to existing systems.

% The idea of informing memory operations is not our primary contribution but rather a mature solution that we adopt to complete our design.

\vspace{1ex}


% \item \textbf{Comparison to AstriFlash (Reviewer A-B)}

% We revised $\S$\ref{sec:related} to discuss this work. 
% \pname is different from AstriFlash in terms of both context and technique. 

% First, with the CXL interface, \pname's CXL-SSD directly appears as CPU-cachable physical memory space, allowing access at cacheline granularity. In contrast, AstriFlash modifies the host CPU hardware to manage the host DRAM as a cache of SSD in order to eliminate OS paging overheads. AstriFlash still treats the SSD as a block device and manages page swapping/migration at 4KB page granularity.

% Second, while AstriFlash only uses SSD as a black box, \pname co-designs the SSD and the host: (1) \pname leverages the SSD controller to trigger context switches based on precise access latency predictions; (2) \pname re-architects the SSD DRAM cache with a write log and a read-write cache to bridge the gap between page-granular flash accesses and the cacheline-granular CXL memory accesses; (3) \pname utilizes the SSD controller to efficiently track hot pages for promotion to host DRAM through an adaptive page migration mechanism.

% Third, compared to the switch-on-miss user-level thread-switching approach in AstriFlash, \pname's coordinated context switch mechanism is more practical and requires less modification to commodity CPUs (i.e., only a new CXL.mem opcode and a new exception type is required). Additionally, \pname supports hiding flash latency with threads/processes from different collocated applications, while AstriFlash can only switch threads within the same process. 

% \vspace{1ex}

\end{enumerate}



\noindent {\large \hlA{\textbf{Reviewer-A}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]


\item \textbf{Comparison to Prior Switch-On-Miss Approaches}

We added the discussion of informing memory operations in $\S$\ref{sec:related}.
\vspace{1ex}

Prior studies~\cite{inform_mem_op:isca96} focused on providing instruction primitives and hardware support for informing memory operations. Inspired by these studies, \pname{} extends the SSD controller to inform the host CPU when a long SSD access happens.
\vspace{1ex}

% We recognize that a coordinated context switch mechanism, rather than the direct switch-on-miss method used in previous studies, is necessary to optimize CXL-SSD performance. This is because the host CPU is unaware of the internal state of the SSD and whether a CXL-SSD memory access latency is long enough. Therefore, \pname lets the SSD controller decide whether to trigger a context switch based on accurate predictions of access latencies. \hl{todo}
% \vspace{1ex}


\item \textbf{Comparison to AstriFlash}

We added the discussion of AstriFlash~\cite{AstriFlash} in $\S$\ref{sec:related}. We also added the performance comparison between \pname{} and AstriFlash in $\S$\ref{sec:eval_comparison} (see ``1. Evaluation Baseline'' in Common Concerns). 

\vspace{1ex}

\pname{} is different from AstriFlash in the following aspects. 
\vspace{1ex}

First, \pname{} is designed for the CXL interface and exploits the byte-addressability of CXL-SSDs. In \pname{}, the CXL-SSD directly appears as a CPU-cachable physical memory space.
In contrast, AstriFlash does not exploit the byte interface of the SSD. AstriFlash modifies the host CPU hardware to manage the host DRAM as a cache of SSD. And AstriFlash still relies on page swapping to access the SSD.
\vspace{1ex}

Second, \pname co-designs the SSD and the host system: (1) \pname leverages the SSD controller to trigger context switches based on precise access latency predictions; (2) \pname re-architects the SSD DRAM cache with a write log to bridge the gap between page-granular flash accesses and the cacheline-granular CXL memory accesses; (3) \pname utilizes the SSD controller to efficiently track hot pages.
In contrast, AstriFlash uses SSD as a black box, which inevitably misses the opportunities to co-optimize the host and the SSD.
\vspace{1ex}

Third, compared to the switch-on-miss user-level thread-switching approach in AstriFlash, \pname's coordinated context switch mechanism is more practical and flexible. It requires less modification to commodity CPUs (i.e., only a new CXL.mem opcode and a new exception type are necessary, compared to new instructions and hardware support for user-level context switching). Additionally, \pname supports hiding flash latency with threads/processes from different collocated applications, while AstriFlash can only switch threads within the same process. 
\vspace{1ex}


\vspace{1ex}

\item \textbf{Evaluation Baseline}

Please see ``1. Evaluation Baseline'' in Common Concerns.
\vspace{1ex}


\item \textbf{Benefits of SSD Write Log}

We clarified the benefits of SSD write log in $\S$\ref{sec:design:write_log}.
\vspace{1ex}

%  I did not quite grasp the value of the log. The results clearly show it has an impact, but logically I’m not sure where that comes from. 
Compared to a traditional page-granular SSD DRAM cache, the write log (1) utilizes the DRAM space more efficiently by caching at a finer granularity, and (2) reduces the flash writeback traffic by providing a larger write coalescing window.
Despite that a page will be first read into the DRAM before it is written to, the write log helps alleviate cache thrashing: upon a cache conflict, a dirty page in \pname{}'s read/write cache can be directly evicted without being written back to the flash, since the dirty cachelines are already recorded by the write log. 
\vspace{1ex}

% The log adds non-negligible complexity and a lot of additional memory lookups and data structure manipulations. What is ultimately the gain?
We quantified the indexing overhead of the write log in $\S$\ref{sec:implementation} and the performance benefit in $\S$\ref{sec:eval_ssd_cache}. The ultimate benefit of the write log greatly outweighs the overhead.
\vspace{1ex}

% It only saves DRAM space if there is a considerable stretch of time during which a page is getting sparsely written without being read at all. How typical is that? If even a single byte from a page is read, the entire page will be placed in DRAM, so the aggregate capacity occupied in DRAM is actually larger (page itself + number of dirty cache blocks in log + log metadata). It's also quite atypical for workloads to atomically write full cache blocks (e.g., using MOVDIR64B) without reading them first. A typical store will anyway require reading the target cache block first, which in turn would require reading the entire corresponding page from SSD.
% Please help me understand why the log's role is so important. Perhaps some data about (i) the time distance between the last read to the last write of a page, and (ii) the time distance between the <first write to a page after the last read> and <last write to a page before the page is written to SSD> will help. A very relevant question is, if every write to the SSD-mapped address space was followed by a clwb, would the log be completely unnecessary?

% The key advantage of the write log is that it provides a much larger coalescing window for data writeback compared to traditional page-level caches. By using DRAM space more efficiently, the write log can buffer more writes in the limited SSD DRAM. This helps absorb redundant updates, significantly reducing flash write traffic, as shown in Figure~\ref{fig:eval_write_traffic}. The write log effectively leverages both temporal and spatial locality: (1) If a cache line is updated multiple times, the log is more likely to retain the latest version in DRAM, reducing unnecessary flushes to flash, unlike traditional caches that may flush it repeatedly due to cache thrashing. (2) If different cache lines in a page are updated at different times, the log can buffer them in DRAM and flush the page only once, while a traditional cache might flush it multiple times.

% \vspace{1ex}


\item \textbf{Clarification on \texttt{clwb}'s Effect on the SSD Write Log}

The \texttt{clwb} instruction only ensures that the cacheline is flushed from the CPU cache to the CXL-SSD.
It will not trigger write log compaction in the SSD, since the data is already considered persistent in the battery-backed SSD DRAM.
\vspace{1ex}


\item \textbf{Comparison to Software-Based Approaches for Tiered Memory Management}

Prior studies have proposed software-based memory management mechanisms for tiered memory systems that orchestrate data placements/movements between a fast-tier and a slow-tier memory.
\pname{} focuses on addressing the performance challenges of CXL-SSDs. It also leverages the tiered memory data management techniques to expand SSD DRAM cache.
\vspace{1ex}

In $\S$\ref{sec:eval}, \pname{}-P represents the baseline that uses tiered memory techniques (i.e., page migration) to manage Base-CSSD.
We also added $\S$\ref{sec:eval_comparison} to evaluate the performance of \pname{} when integrating different page migration mechanisms into \pname{} (see ``1. Evaluation Baseline'' in Common Concerns). 

% However, there is a key difference: in state-of-the-art software-based tiered memory solutions (e.g., TPP, Thermostat), data placement is managed by the host OS. In contrast, \pname relies on the SSD controller to track page access counts and decide which pages to migrate to the host. In this specific context, we believe tracking hot pages using the SSD controller is a simple and efficient approach, as it incurs negligible overhead on the critical path. Conversely, page temperature detection in the OS typically requires page sampling, which adds overhead, since normal memory accesses are transparent to the OS.

% Other software-based tiered memory solutions can also be applied to \pname. We added the TPP approach as a new baseline in $\S$\ref{sec:eval} and compared its performance with the original \pname design.

\vspace{1ex}


\item \textbf{Peak Throughput of Write Log Operations}

We added the peak throughput of our FPGA SoC prototype implementation in $\S$\ref{sec:implementation}.
Our prototype uses FPGA logic to implement data structure lookups. It can achieve 11.93/9.37 GB/s for cacheline reads/writes.
\vspace{1ex}


\item \textbf{Modeling of Page Migrations}

We revised $\S$\ref{sec:implementation} to elaborate on how we model page migrations in our simulator.
\vspace{1ex}

We implement the PLB ($\S$\ref{subsec:migration}) in our simulator and let the CPU issue CXL memory requests to the SSD to migrate a page in the background. To simulate the side effects of page migration, we perform a TLB shootdown for all cores when a page finishes migration.
\vspace{1ex}


\item \textbf{Data Persistence in \pname{}}

We added the discussion on the data persistence support of \pname{} in $\S$\ref{sec:discussion}.
\vspace{1ex}

\pname{} supports data persistence by providing the option for the user to pin the memory pages %\hl{(how??)} 
in the CXL-SSD, such that these pages will not be migrated to the host.
As the main objective of \pname{} is to expand the main memory capacity with CXL-SSDs, \pname{} by default allows page migration to the host to improve performance when the user application does not have persistence requirements.
% If the user wants to ensure persistence for specific data, \pname provides the option to pin the data within the device, preventing it from being migrated to the host. However, in the context of using CXL-SSDs to scale main memory capacity at a lower cost (which remains volatile), we expect that most applications will not have persistence requirements.
\vspace{1ex}


\item \textbf{Clarification on the Description of CXL Device Types}

We revised $\S$\ref{sec:cxl_background} to provide a more accurate description of CXL device types.
\vspace{1ex}


\item \textbf{Clarification of Exception Handling}

\pname{} leverages the existing hardware exception mechanism in modern CPUs to eliminate false-positive context switches without extra hardware cost, since modern processors by default delay the exception handling to the retire stage.
% \pname{} leverages the existing hardware exception mechanism in modern CPUs, which by default prevents speculative load/store and hardware prefetch operations to trigger the \pname{} Long Delay exception even if they cause SSD DRAM misses and the SSD controller returns a CXL No Data Response message with the \pname{}-Delay opcode.
% , the \pname Long Delay Exception is indeed handled the same as other exceptions.
We revised $\S$\ref{sec:design:context_switch} to clarify this.
\vspace{1ex}


\item \textbf{Possibility of DoS Attacks}

\pname{} will not introduce new opportunities for exploiting DoS attacks.
\vspace{1ex}

To carry out the described DoS attack, the attacker needs to rapidly generate a large amount of SSD DRAM misses such that the victim thread's data will be evicted from the SSD DRAM before that thread is rescheduled and actually accesses the data.
% It should overwhelm the SSD DRAM cache during the interval after the victim thread triggers a context switch on the first SSD DRAM miss and before that thread is rescheduled.
However, this is unlikely because each of the attacker's threads will be context-switched upon its first SSD DRAM miss, preventing further misses until the requested page is loaded into SSD DRAM. This means the attacker must launch thousands or even more threads to overwhelm the SSD DRAM cache, since each thread can only trigger one SSD DRAM miss at a time. With such a huge number of threads, this will be considered as a DoS attack against the CPU, which is out of the scope of \pname{}.
% At the same time, the OS's CFS scheduling policy ensures that the victim thread is quickly rescheduled.
\vspace{1ex}


\item \textbf{SSD Latency Prediction}

It is common for modern SSD controllers to use a FIFO scheduling policy to serve SSD requests~\cite{ssd-book}.
In Algorithm~\ref{algo:threshold_trigger_policy}, we predict the latency using information from the flash channel queues (Lines 3-4). While the controller may reorder incoming requests to enhance performance (e.g., prioritizing read requests over write requests since flash writes have higher latency than reads), once requests are enqueued, they will be issued in FIFO order.
% \pname{} can also support other scheduling policies as long as the SSD firmware developer knows how to predict the flash access latency for their specific policy.
\vspace{1ex}


\item \textbf{Stacked Bar Figure for Table IV}

Thanks for the suggestion. We replaced the original Table IV with Figure~\ref{fig:breakdown_access}.
\vspace{1ex}

\end{enumerate}

\noindent {\large \hlB{\textbf{Reviewer-B}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]


\item \textbf{Impact of Context Switching on SSD Latency Under Parallel Threads}

We revised $\S$\ref{sec:eval_context_switch} to discuss the impact of context switching on SSD latency as we increase the number of threads. Due to the space limitation, we added the detailed experimental numbers in Appendix~\ref{appendix:eval_ctx_switch_ssd_latency} and Figure~\ref{fig:eval_ltcy_vary_threads}. 
\vspace{1ex}

With more threads, the end-to-end latency of flash accesses may also increase due to queuing delays.
However, the end-to-end performance is still better since the SSD bandwidth utilization is higher.
\vspace{1ex}


\item \textbf{Research Contributions of \pname{}}

Please see ``2. Research Contributions" in Common Concerns.
\vspace{1ex}


\end{enumerate}


\noindent {\large \hlC{\textbf{Reviewer-C}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Considering Garbage Collection in SSD Latency Prediction}

We revised $\S$\ref{sec:design:context_switch} to clarify how \pname deals with GCs.
\vspace{1ex}

Although the timing of garbage collection (GC) is hard to predict, the SSD controller can detect whether an incoming request is blocked by an ongoing GC. If a request is blocked by an ongoing GC, \mbox{\pname} will immediately trigger a context switch, as GCs typically last for milliseconds. While the GC process will block the issuing of requests in the queue, 
%issue internal flash operations that affect the queuing delay of regular requests, 
its impact is already considered in the latency prediction algorithm by querying the flash channel queue status.
\vspace{1ex}


\item \textbf{Write Log Compaction}

We revised $\S$\ref{sec:design:write_log} to provide more details for write log compaction.
\vspace{1ex}

\pname maintains a double-buffered log to avoid blocking incoming requests and performs the compaction in the
background.
When one log becomes full, \mbox{\pname{}} triggers the log compaction process and switches to a new log. The SSD’s channel-level parallelism is leveraged by distributing writes across multiple channels.
\vspace{1ex}


\item \textbf{Page Migration}

\pname{} utilizes the host memory to expand the SSD DRAM cache, because the SSD DRAM is not large enough to hide the high flash access latency, as shown by our study in $\S$\ref{sec:bkg_motiv}.
Therefore, similar to prior studies on tiered memory systems, we develop the adaptive page migration mechanism to manage data movement and placement across the fast host DRAM and slow SSD device.
This does not contradict the purpose of the CXL design, and we use the CXL-SSD as a Type-3 CXL memory expansion device.
\vspace{1ex}

% Our goal is to provide a full-system solution to efficiently use CXL-based memory semantic SSDs to expand the main memory capacity. Therefore, besides optimizing CXL-SSD itself, we also want to best utilize the host main DRAM memory. This does not contradict the purpose of CXL design.

% Our page migration mechanism brings decent benefits, reflected by the \pname-P baseline
Please refer to the performance of \pname-P in our evaluation ($\S$\ref{sec:eval_overall}) for the benefits of adaptive page migration.
\vspace{1ex}


\item \textbf{Number of Threads in the Traces}

We run each workload multiple times with different numbers of threads. In each run, we collect a separate trace for each thread. We ensure that all traces represent the same section of the program.
We revised $\S$\ref{sec:exp_setup} to clarify this.
\vspace{1ex}


\item \textbf{Clarification on the SSD Simulator}

We modified MacSim and SimpleSSD to implement \pname{}.
We revised $\S$\ref{sec:implementation} to clarify this.
\vspace{1ex}


\item \textbf{Clarification on the Base-CSSD Baseline}

In our evaluation, Base-CSSD represents the state-of-the-art CXL-based SSD device that incorporates all optimizations developed by the two cited works~\cite{atc-cxlssd,hello-bytes}.
We revised $\S$\ref{sec:exp_setup} to clarify this.
\vspace{3ex}


\item \textbf{Clarification on the FPGA Prototype}

We revised $\S$\ref{sec:implementation} to clarify how to implement the FPGA SoC prototype.
\vspace{1ex}

We implemented the SSD controller functionalities of \pname{} on an FPGA SoC board and used it to verify the performance model used in our simulator. We did not directly use the FPGA SoC prototype to evaluate the end-to-end performance of \pname{}, since \pname{} requires host CPU hardware changes (e.g., to trigger the \pname{} Long Delay Exception), and we did not have access to a real CXL-capable FPGA board.
\vspace{1ex}

\end{enumerate}


\noindent {\large \hlD{\textbf{Reviewer-D}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Swap-Over-NVMe Baseline}

Please see ``1. Evaluation Baseline'' in Common Concerns.
\vspace{1ex}


\item \textbf{Evaluation Methodology}

To implement \pname's coordinated context switch mechanism, we need to slightly modify the CPU hardware (to handle context switch requests) and the CXL controller hardware (to support the new \texttt{\pname-Delay} opcode). Therefore, we opted for a simulation-based evaluation.
To ensure accurate simulation, we collected real instruction traces using Intel's PIN\cite{pin} tool and replayed them on a cycle-accurate simulator developed upon widely-used simulators~\cite{macsim,simplessd:micro18}.
We also prototyped the SSD-side design components of \pname{} on a Xilinx MPSoC board and verified the performance model used in our simulator.
Please see $\S$\ref{sec:implementation} and $\S$\ref{sec:exp_setup} for our implementation and evaluation methodology.
\vspace{1ex}


\item \textbf{Discussion about PCI vs. CXL}

We revised $\S$\ref{sec:cxl_background} to provide a more accurate description of CXL and memory expansion, including the capability of different CXL protocols and the definition of CXL device types.

The design of \pname{} can work with the traditional PCIe interface if the host CPU supports cachable PCIe MMIO region. In this paper, we focus on CXL devices. 
%since the commodity x86 CPUs do not support cachable PCIe MMIO.
\vspace{1ex}


\item \textbf{Clarification on SSD Latency Parameters in Evaluation}

The Read/Program/Erase ($t_\text{R}$/$t_{\text{Prog}}$/$t_{\text{BERS}}$) parameters represent the latencies of NAND flash operations, i.e., the time required to read or program a page, or erase a block on a flash chip.

We revised $\S$\ref{sec:eval_ssd_cache} to clarify the latency components. The CXL-SSD access latency observed by the host CPU consists of the following components: (1) the SSD DRAM cache indexing time (72 ns for the write log, 49 ns for the data cache, see \mbox{$\S$\ref{sec:implementation}}), (2) the SSD DRAM access time (based on the timing in Table \mbox{\ref{tab:exp_setup}}), and (3) the flash chip latency (see Table \mbox{\ref{tab:exp_setup}}) in case of an SSD DRAM miss.
Please see Figure~\ref{fig:eval_amat_breakdown} for the end-to-end latency breakdown.
\vspace{1ex}


\item \textbf{Clarification on Figure~\ref{fig:context_switch}}

Thanks for pointing this out. We have updated Figure~\ref{fig:context_switch} to the correct version. After the SSD sends a \pname{}-Delay response to the host, the CPU cache will not be updated. When the original thread is scheduled back, the previously missed memory instruction will be executed again to fetch the data from the SSD DRAM.
\vspace{1ex}


\item \textbf{SSD Controller Occupancy During Log Compaction}

The write log compaction will only dominate one SSD controller core during the compaction period (146 $\mu s$ on average). Given that the indexing of the write log and data cache can be accelerated by custom hardware and requires minimal CPU resources (see our FPGA SoC prototype in $\S$\ref{sec:implementation}), the log compaction will not compete with regular SSD access requests for the CPU resource in the SSD controller.
\vspace{1ex}

% \item \textbf{Revise Figure Bars}

% Thanks for your suggestion. We polished our bar plots.
% \vspace{1ex}


\item \textbf{Presentation Quality}

We have taken an editorial pass on our paper to improve the presentation quality, including revising the figures and fixing the incomplete reference.
\vspace{3ex}


\end{enumerate}


\noindent {\large \hlE{\textbf{Reviewer-E}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]


\item \textbf{Comparison With State-of-the-Art CXL-SSD}

In our evaluation, the \basename{} baseline represents the state-of-the-art (SOTA) CXL-based SSD device that incorporates all optimizations developed by recent works~\cite{atc-cxlssd,hello-bytes}, as described in $\S$\ref{sec:exp_setup}.
We also added new baselines that utilize host memory as suggested by other reviewers (see ``Evaluation Baseline'' in Common Concerns).
\vspace{1ex}

% We also added stronger baselines that utilized host memory as reviewers suggested in our revised paper. Please see ``Evaluation Baseline (Reviewer-A-D-E-F)" in Common Concerns.


\item \textbf{Data Management Granularity of SOTA CXL-SSD}

To the best of our knowledge, no prior works on CXL-SSDs have addressed the granularity mismatch between cacheline-level CXL memory accesses and page-level flash accesses. They mostly focused on how to optimize the host hardware/software to better utilize the CXL-SSD device.
For the two state-of-the-art (SOTA) CXL-SSD designs~\cite{atc-cxlssd,hello-bytes} cited in our evaluation, they both use the default page-level DRAM cache inside the SSD.
\pname{} examines the internal SSD design and co-optimizes the host system and the SSD to address the access granularity mismatch.
\vspace{1ex}

\item \textbf{Presentation Quality}

We have taken an editorial pass on our paper to improve the presentation quality, including revising the X-axis labels in Figure~\ref{fig:eval_amat_breakdown} (originally Figure 16).
\vspace{1ex}


\end{enumerate}



\noindent {\large \hlF{\textbf{Reviewer-F}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Comparison to Other Tiered Memory Solutions}

Please see ``1. Evaluation Baseline'' in Common Concerns.
\vspace{1ex}


\item \textbf{Clarification on Software-based Memory Management}

% Software prefetching, Swapping and HMM are all not enabled in this work. 
% There is no software based tiered memory management enabled in both motivation and baselines. 
For the motivation experiments in $\S$\ref{sec:motivation} and the \basename{} baseline in $\S$\ref{sec:eval}, we did not enable any software-based memory placement/swapping optimizations. All application data are placed in either the host DRAM or the CXL-SSD.
\vspace{1ex}

In $\S$\ref{sec:eval}, the \pname{}-P baseline represents a system that uses software-based memory management techniques on CXL-SSD.
In our revised paper, we also added $\S$\ref{sec:eval_comparison} and Figure~\mbox{\ref{fig:comparision_tiered}} to evaluate \pname{}'s performance when integrating the tiered/heterogeneous memory management techniques from prior studies. Please also see ``1. Evaluation Baseline'' of Common Concerns.
\vspace{1ex}


\item \textbf{Clarification on Scheduling vs. Context Switch}

We revised $\S$\ref{sec:design:context_switch} and added the execution time breakdown in Figure~\ref{fig:eval_context_switch_policy}.
\vspace{1ex}

The three policies deliver similar performance, because the threads are mainly bounded by memory I/O, and all three policies ensure that threads have equal or similar opportunities to issue memory requests to the SSD.
% \hl{This improves the end-to-end performance by improving the SSD bandwidth utilization with multi-threading} (see $\S$\ref{sec:eval_context_switch}). \hl{what is this for?}
\vspace{1ex}

The reason why all threads are I/O-bound even with the context switch mechanism is due to the performance gap between the fast computing speed of the host CPU and the long latency of NAND flash. Exploring SSD-side scheduling may slightly reduce the SSD I/O latency but cannot fundamentally address this issue.
\vspace{1ex}


\item \textbf{Discussion on SkyByte and NUMA System}

We added the discussion of how \pname{} works with NUMA architecture in $\S$\ref{sec:discussion}.
\vspace{1ex}

\pname{} uses the same context switch threshold for all NUMA nodes. The flash access latency ($\mu$s-level) is much higher than the inter-socket communication latency (less than 100 ns), so tuning the threshold for different NUMA nodes has limited performance benefit. 
\vspace{1ex}

For page migration, \pname{} promotes the page to the main memory of the home node of the CXL-SSD, and leverages existing OS NUMA balancing mechanisms to further move this promoted page to other NUMA nodes when applicable. 
\vspace{1ex}


\item \textbf{Discussion on How SkyByte Handles Multiple Page Sizes}

We added the discussion of how \pname handles multiple page sizes in $\S$\ref{sec:discussion}.
\vspace{1ex}

When the host OS receives the migration request (MSI-X interrupt) from the SSD with a 4KB-page address, it first checks whether this address belongs to a huge page. If it does, the host OS allocates a physical huge page in the host DRAM, and migrates the entire page by copying all 4KB data chunks from the SSD. Once the migration finishes, the host sends a custom NVMe command to notify the SSD to remove all corresponding 4KB chunks from its internal DRAM caches.
\vspace{1ex}

To migrate a huge page, the PLB needs to track all cachelines in the huge page.
However, tracking all 32768 cachelines in a 2MB page requires a 4KB bitmap per PLB entry.
To reduce the hardware cost of PLB, we extend the original PLB into a two-level structure.
% The first-level entry contains a 64B bitmap that indicates whether a 4KB chunk in a 2MB page has been migrated. The second-level entry contains an 8B bitmap to track which cachelines in a 4KB chunk have been migrated.
% Instead of tracking all cachelines in the 2MB page simultaneously,
The PLB migrates the huge page chunk-by-chunk, and it only needs one first-level entry and one second-level entry to track the migration progress of a 2MB page.
\vspace{1ex}

% When the host receives the migration request from the SSD with a 4KB-page address, it first checks whether this address belongs to a larger page, and then migrates all relevant 4KB data chunks from SSD to host DRAM. After migration, the SSD is notified to remove all the corresponding 4KB pages from its internal cache.
% \vspace{1ex}

% To accommodate larger pages like 256KB, the promotion look-aside buffer (PLB) needs to be extended to a multi-level table to track and manage ongoing migrations efficiently.
% \vspace{1ex}


\item \textbf{Clarification on Hardware Support for Tiered Memory}

NVMs like Intel Optane DIMM are typically deployed in two modes: memory mode and app-direct mode.
\vspace{1ex}

In memory mode, the CPU hardware manages the host DRAM as an inclusive, 64B-granular, direct-mapped cache for the NVM. 
% In contrast, in the context of CXL-SSDs, the host DRAM cannot directly be used as an inclusive cache for SSD, because the CXL.mem protocol maps the host DRAM and CXL-SSD as two exclusive parts of physical memory. However, if one modifies the host memory controller hardware, it's also possible to use DRAM as a hardware-managed cache for CXL-SSD.
In the context of CXL-SSD, this approach will suffer from the long flash access latency (see $\S$\ref{sec:bkg_motiv}) upon a DRAM cache miss. The direct-mapped cache may also suffer from cache thrashing overheads.
In $\S$\ref{sec:eval_comparison}, we added a more relevant and more competitive baseline AstriFlash-CXL, which is a hardware-managed tiered memory system for SSD, and compared its performance with \pname{}. Please also see ``2. Comparison to AstriFlash'' of Reviewer-A.
\vspace{1ex}

% \textit{OS-managed NUMA memory.} 
In app-direct mode, the NVM is exposed to the OS software as a separate physical memory region (the same as a Type-3 CXL device). The OS software explicitly manages the NVM memory. Please see ``2. Clarification on Software-based Memory Management'' of Reviewer-F for discussion on software-based tiered memory management.
\vspace{1ex}
% such as through the kernel non-uniform memory (NUMA) management and let all processors treat the NVM as non-local memory. Existing works have proposed many software-based page migration mechanisms (e.g., TPP\mbox{\cite{tpp:asplos2023}}).

% This approach can also be applied to CXL-SSDs. In $\S$\ref{sec:eval_comparison}, we added the baseline \mbox{\pname-CT} 
%  and \mbox{\pname-WCT} to represent such an design and compared its performance with \pname{}.
% \vspace{1ex}


\item \textbf{Intel Flat Memory Mode}

Intel Flat Memory Mode is a hardware-managed memory tiering mechanism that orchestrates data movements between the fast main memory and the slow CXL-memory at cacheline granularity. It does not optimize for CXL-SSDs and will suffer from high flash access latency.
\pname{} addresses the performance challenges of CXL-based SSDs and co-designs the host and the SSD to manage data across memory tiers.
% , especially (1) the latency of CXL-SSD causes severe processor pipeline stalls, and (2) the mismatch in access granularity causes DRAM space waste and write traffic amplification.
We added the citation of Intel Flat Memory Mode in $\S$\ref{sec:related}.
\vspace{1ex}
% and pave the way for using memory semantic SSDs to expand memory capacity. 



\item \textbf{Presentation Quality}

We have taken an editorial pass on our paper to improve the presentation quality.
\vspace{1ex}


\end{enumerate}



\noindent {\large \hlG{\textbf{Reviewer-G}}}
% \vspace{0.5ex}

\begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*]

\item \textbf{Clarification on OS Implementation}

Please see $\S$\ref{sec:design:context_switch} for how the existing OS needs to be modified to support the \pname{} Long Delay Exception, and $\S$\ref{subsec:migration} for how the OS supports adaptive page migration.
\vspace{1ex}

Since \pname{} requires host CPU hardware changes (e.g., to trigger the \pname{} Long Delay Exception), and CXL hardware changes (e.g., to support the new \texttt{SkyByte-Delay} opcode), 
%it's impractical for us to evaluate it with a real OS prototype. Therefore, 
we opted for a simulation-based evaluation. %and did not implement the design in an existing OS.
\vspace{1ex}


\item \textbf{Evaluation Methodology for the OS Overheads}

% The effect of OS code to a simulated application may include the followings: 
During the execution of an application, the OS is mainly involved in the following two cases. (1) Context switches: as described in $\S$\ref{sec:implementation}, we measured the context switch overhead with an Intel E5 CPU under real systems, and set our simulator timing model accordingly. (2) Page migration: when a page finishes migration, there will be a TLB shootdown for the entire application after the OS updates the page table entry. We modified MacSim to perform a TLB shootdown for all cores in this case. We revised $\S$\ref{sec:implementation} to clarify this. 
\vspace{1ex}


\item \textbf{Clarification on the FPGA Prototype}

We revised $\S$\ref{sec:implementation} to elaborate on the FPGA SoC prototype. We implemented the SSD controller functions of \pname{} on the FPGA SoC board and used it to verify the performance model used in our simulator, including the log and data cache indexing latency and the log compaction overhead.
\vspace{1ex}

\end{enumerate}
